DriveGPT4: Interpretable End-to-end Autonomous Driving via Large Language Model

Multimodal large language models (MLLMs) have emerged as a prominent area of interest within the research community, given their proficiency in handling and reasoning with non-textual data, including images and videos. This study seeks to extend the application of MLLMs to the realm of autonomous driving by introducing DriveGPT4, a novel interpretable end-to-end autonomous driving system based on LLMs. Capable of processing multi-frame video inputs and textual queries, DriveGPT4 facilitates the interpretation of vehicle actions, offers pertinent reasoning, and effectively addresses a diverse range of questions posed by users. Furthermore, DriveGPT4 predicts low-level vehicle control signals in an end-to-end fashion.These advanced capabilities are achieved through the utilization of a bespoke visual instruction tuning dataset, specifically tailored for autonomous driving applications, in conjunction with a mix-finetuning training strategy. DriveGPT4 represents the pioneering effort to leverage LLMs for the development of an interpretable end-to-end autonomous driving solution. Evaluations conducted on the BDD-X dataset showcase the superior qualitative and quantitative performance of DriveGPT4. Additionally, the fine-tuning of domain-specific data enables DriveGPT4 to yield close or even improved results in terms of autonomous driving grounding when contrasted with GPT4-V.

==> figures/fig_add_ex.tex <==
\begin{figure}[!h]
  \centering
    \includegraphics[width=0.49\linewidth]{imgs/ex1.pdf}
     \includegraphics[width=0.49\linewidth]{imgs/ex2.pdf}
     \vspace{-5pt}
  \caption{Conversations generated by DriveGPT4. In these examples, it is tested on the BDD-X testing set.}
  \label{add_example_1}
\vspace{-5pt}
\end{figure}

\begin{figure}[!h]
  \centering
    \includegraphics[width=0.49\linewidth]{imgs/ex3.pdf}
     \includegraphics[width=0.49\linewidth]{imgs/ex4.pdf}
     \vspace{-5pt}
  \caption{Conversations generated by DriveGPT4. In these examples, it is tested on the BDD-X testing set.}
  \label{add_example_2}
\vspace{-5pt}
\end{figure}

\begin{figure}[!h]
  \centering
    \includegraphics[width=0.49\linewidth]{imgs/ex5.pdf}
     \includegraphics[width=0.49\linewidth]{imgs/ex6.pdf}
     \vspace{-5pt}
  \caption{Conversations generated by DriveGPT4. In these examples, it is tested on the BDD-X testing set.}
  \label{add_example_3}
\vspace{-5pt}
\end{figure}

\begin{figure}[!h]
  \centering
    \includegraphics[width=0.49\linewidth]{imgs/ex7.pdf}
     \includegraphics[width=0.49\linewidth]{imgs/ex8.pdf}
     \vspace{-5pt}
  \caption{Conversations generated by DriveGPT4. In these examples, it is tested on the BDD-X testing set.}
  \label{add_example_4}
\vspace{-5pt}
\end{figure}

==> figures/fig_evaluate_consistency.tex <==
\begin{figure}[!h]
  \centering
    \includegraphics[width=0.9\linewidth]{imgs/consistency.pdf}
  \caption{Examples of consistency evaluation. In these examples, we prompt ChatGPT to explain its evaluation scores.}
  \label{example_gpt_consistency}
\vspace{-10pt}
\end{figure}

==> figures/fig_gpt_evaluate_explain.tex <==
\begin{figure}[!h]
  \centering
    \includegraphics[width=0.7\linewidth]{imgs/gpt_evaluate_example_explain.pdf}
  \caption{Evaluation results comparison. In this example, we provide texts generated by ChatGPT to explain its evaluation scores.}
  \label{example_gpt_explain}
\vspace{-10pt}
\end{figure}

==> figures/fig_gpt_metric.tex <==
\begin{figure}[t]
  \centering
    \includegraphics[width=0.8\linewidth]{imgs/gpt_example.pdf}
  \caption{Example of evaluation metrics. Compared to conventional metrics, the score generated by ChatGPT is more reasonable and convincing for evaluation.}
  \label{gpt_metric}
\vspace{-15pt}
\end{figure}

==> figures/fig_video_tokenizer.tex <==
\begin{figure}[t]
  \centering
    
    \includegraphics[width=\linewidth]{imgs/video_tokenizer.pdf}
    \vspace{-15pt}
  \caption{Architecture of the video tokenizer.}
  \label{tokenizer}
\vspace{-15pt}
\end{figure}

==> figures/multi_head.tex <==
\begin{figure}[t]
  \centering
    \includegraphics[width=\linewidth]{imgs/multi_head.pdf}
    % \vspace{-20pt}
  \caption{DriveGPT4 with multi-head design. In conventional LLM, a number like "1.98" would be split into "1", ".", "9", and "8", and the LLM would process them as four separate characters instead of a single numerical value. This counter-intuitive approach may affect performance. In DriveGPT4, the number "1.98" is processed as a single entity during training. During inference, if the text head outputs $<$number\_token$>$, the output of the control head (e.g., 0.35 in this example) is tokenized into separate tokens as history to maintain consistency with LLM pre-training.}
  \label{multi-head design}
\vspace{-10pt}
\end{figure}

==> tables/fiexd_qas.tex <==
\begin{table*}[!h]\centering
\begin{minipage}{0.7\columnwidth}\vspace{0mm}    \centering
\begin{mybox}{purple}
    \centering
   
    %  \hspace{-10mm}
      \footnotesize
    \begin{tabular}{p{0.97\columnwidth} c}

    What is the current action of this vehicle? \\
    What is the vehicle doing right now in this video?\\
    What action is the vehicle performing in this video at the moment?\\
    Can you describe the vehicle's current activity in this video?\\
    What's happening with the vehicle in this video right now?\\
    At this moment in the video, what is the vehicle engaged in?\\
    What can you observe the vehicle doing in this video currently?\\
    How is the vehicle behaving at this point in the video?\\
    What is the ongoing action of the vehicle in the video?\\
    In this video, what action is the vehicle involved in at present?\\
    Describe the current state of the vehicle in this video.
    \end{tabular}
\end{mybox}
\vspace{-4mm}
\caption{Question set $Q_a$.
}
    \label{tab:qa}
    \vspace{-5pt}
\end{minipage}

\end{table*}


\begin{table*}[!h]\centering
\begin{minipage}{0.7\columnwidth}\vspace{0mm}    \centering
\begin{mybox}{purple}
    \centering
   
    %  \hspace{-10mm}
      \footnotesize
    \begin{tabular}{p{0.97\columnwidth} c}

    Why does this vehicle behave in this way?\\
    What is the reason behind this vehicle's behavior?\\Can you explain the cause of this vehicle's actions?\\What factors contribute to the way this vehicle is behaving?\\What's the rationale behind this vehicle's behavior?\\Why is the vehicle acting in this particular manner?\\What prompted the vehicle to behave like this?\\What circumstances led to this vehicle's behavior?\\What is the underlying cause of this vehicle's actions?\\For what reason is the vehicle exhibiting this behavior?\\What's driving the vehicle to behave in this way?
    \end{tabular}
\end{mybox}
\vspace{-4mm}
\caption{Question set $Q_j$.
}
    \label{tab:qj}
    \vspace{-5pt}
\end{minipage}

\end{table*}


\begin{table*}[!h]\centering
\begin{minipage}{0.7\columnwidth}\vspace{0mm}    \centering
\begin{mybox}{purple}
    \centering
   
    %  \hspace{-10mm}
      \footnotesize
    \begin{tabular}{p{0.97\columnwidth} c}

    Predict the speed and turning angle of the vehicle in the next frame.\\Foresee the speed and turning angle of the vehicle in the following frame.\\Anticipate the speed and turning angle of the vehicle in the subsequent frame.\\Estimate the speed and turning angle of the vehicle in the next frame.\\Project the speed and turning angle of the vehicle in the upcoming frame.\\Forecast the speed and turning angle of the vehicle in the ensuing frame.\\Envision the speed and turning angle of the vehicle in the next frame.\\Expect the speed and turning angle of the vehicle in the following frame.\\Presume the speed and turning angle of the vehicle in the subsequent frame.\\Prognosticate the speed and turning angle of the vehicle in the next frame.\\Calculate the speed and turning angle of the vehicle in the upcoming frame.
    \end{tabular}
\end{mybox}
\vspace{-4mm}
\caption{Question set $Q_c$.
}
    \label{tab:qc}
    \vspace{-5pt}
\end{minipage}

\end{table*}

==> tables/tab_consistency.tex <==
\begin{table}[!h]
 % \vspace{-10pt}
  \caption{Evalution results of prediction consistency. }
   
  \renewcommand\tabcolsep{10pt} 
  \small
  \label{results_consistency}
  \centering
\begin{tabular}{lc}
\toprule
    Method & ChatGPT$\uparrow$ \\ 
    \midrule
    ADAPT & 79.40\\
    \midrule
    DriveGPT4 & 80.69\\
    \bottomrule
  \end{tabular}
  \vspace{-7pt}

\end{table}




==> tables/tab_evaluate.tex <==
\begin{table*}[!h]\centering
\begin{minipage}{0.9\columnwidth}\vspace{0mm}    \centering
\begin{mybox}{purple}
    \centering
   
    %  \hspace{-10mm}
      \footnotesize
    \begin{tabular}{p{0.97\columnwidth} c}

    Now there are some descritions about a driver driving a vehicle. The ground truth description is: \textcolor{Q_rgb}{\{GT label\}}. The description generated by deep learning model is: \textcolor{Q_rgb}{\{Prediction\}}. \\ \\
    Give me an evaluation score about the predicted description. The score should range from 0 to 1. Larger score means better description. The score should be a float number with 2 decimal places. For example, 0.51, 0.99, 0.00, 0.76, etc.\\ \\ 
    You should first give me the score number, and then provide explanations for your score number.
    \end{tabular}
\end{mybox}
\vspace{-4mm}
\caption{Prompts for response text evaluation. Compared with conventional metrics, the score generated by ChatGPT is more reasonable and convincing.
}
    \label{tab:evlauate prompt explain}
    \vspace{-5pt}
\end{minipage}

\end{table*}



==> tables/tab_gpt_consistency.tex <==
\begin{table*}[t!]\centering
\begin{minipage}{0.9\columnwidth}\vspace{0mm}    \centering
\begin{mybox}{purple}
    \centering
   
    %  \hspace{-10mm}
      \footnotesize
    \begin{tabular}{p{0.97\columnwidth} c}

    Here are texts describing a vehicle action and its control signals. \\ \\
        Positive examples: \\
        1. [The car is stopped","because the light is red.","Speed: 0.21; Turning angle: 0.0"]. \\
        2. ["The car is turning left","because the light is green.","Speed: 5.47; Turning angle: -89.59"].\\ \\
        Negative examples: \\1. [The car is turning left","because the light is green.","Speed: 5.47; Turning angle: 89.59"]: The car is tunring left, so that the turning angle should be negative, thus the control and the text are not consistent. \\
        2. [The car is stopped","because the light is red.","Speed: 10.21; Turning angle: 0.0"]: The car should be stopped, but the speed is very high, which is not correct. 
                        \\ \\
        Now, please provide a score ranging from 0-1 to measure the consistency of the control and text of the following case. Note that you should only provide a score figure, and no other text is allowed.\\
        \textcolor{Q_rgb}{\{Predictions to be evaluated\}}
    \end{tabular}
\end{mybox}
\vspace{-4mm}
\caption{Prompts for prediction consistency evaluation. 
}
    \label{tab:eval_consistency}
    \vspace{-5pt}
\end{minipage}

\end{table*}



==> tables/tab_prompt_vit.tex <==
\begin{table*}[!h]\centering
\begin{minipage}{0.9\columnwidth}\vspace{0mm}    \centering
\begin{mybox}{purple}
    \centering
   
    %  \hspace{-10mm}
      \footnotesize
    \begin{tabular}{p{0.97\columnwidth} c}

    There is a 8-frame video recording a drive driving a vehicle. \textcolor{Q_rgb}{\{BDD-X captions\}}. There are some exclusive privilege information, but you cannot mention them in your generated question answering. 1. Objects in each frame of the video: \textcolor{Q_rgb}{\{objects\}}; 2. The speed (m/s) of the vehicle in each frame :\textcolor{Q_rgb}{\{speed\}}. The turning angle (degree) of the vehicle in each frame :\textcolor{Q_rgb}{\{turning angle\}}.\\ \\
    
    
    Design a conversation between you and a person asking about this video. The answers should be in a tone that a visual AI assistant is seeing the video and answering the question.
    Ask diverse questions and give corresponding answers.\\ \\

    Include questions asking about the visual content of the video, including the ego vehicle, traffic light, turning direction, lane change, surrounding objects, objects spatial relations, etc. Only include questions that have definite answers: \\
    (1) one can see the content in the video that the question asks about and can answer confidently;
    (2) one can determine confidently from the video that it is not in the video.
    Do not ask any question that cannot be answered confidently. \\
    Do not contain specific numbers in the questions, e.g., normalized coordinates, speed value, turning angle. \\ \\
            
    Also include complex questions that are relevant to the content in the video, for example, asking about background knowledge of the objects in the video, asking to discuss about events happening in the video, etc. Again, do not ask about uncertain details.
    Provide detailed answers when answering complex questions. For example, give detailed examples or reasoning steps to make the content more convincing and well-organized. You can include multiple paragraphs if necessary.
\\ \\
    The conversation should be 3 turns. Make the answer concise and accurate.
    \end{tabular}
\end{mybox}
\vspace{-4mm}
\caption{Prompts for visual instruction generation. ChatGPT can access privileged information like ground truth BDD-X captions, object boxes, vehicle speeds and turning angles.
}
    \label{tab:vit prompt}
    \vspace{-5pt}
\end{minipage}

\end{table*}

